Computational MRI with Physics-based Constraints: Application to Multi-contrast and Quantitative Imaging

Compressed sensing takes advantage of low-dimensional signal structure to reduce sampling requirements far below the Nyquist rate. In magnetic resonance imaging (MRI), this often takes the form of sparsity through wavelet transform, finite differences, and low rank extensions. Though powerful, these image priors are phenomenological in nature and do not account for the mechanism behind the image formation. On the other hand, MRI signal dynamics are governed by physical laws, which can be explicitly modeled and used as priors for reconstruction. {1}These explicit and implicit signal priors can be synergistically combined in an inverse problem framework to recover sharp, multi-contrast images from highly accelerated scans. Furthermore, the physics-based constraints provide a recipe for recovering quantitative, bio-physical parameters from the data. This article introduces physics-based modeling constraints in MRI and shows how they can be used in conjunction with compressed sensing for image reconstruction and quantitative imaging. We describe model-based quantitative MRI, as well as its linear subspace approximation. We also discuss approaches to selecting user-controllable scan parameters given knowledge of the physical model. We present several MRI applications that take advantage of this framework for the purpose of multi-contrast imaging and quantitative mapping.

==> old_1_intro.tex <==
\mysection{Introduction}
Magnetic resonance imaging (MRI) takes advantage of spin angular momentum present
in atoms with an odd number of protons and/or neutrons. These MR-relevant nuclei,
called \textit{spins}, can be manipulated in the presence of different magnetic fields to produce a
detectable signal \cite{bib:wrightspm}. Quite serendipitously, hydrogen spins in water are abundantly found in
biological tissue, making MRI especially suitable for non-invasive medical imaging. 
MRI is used to visualize soft tissue contrast, capture motion, track functional and behavioral
dynamics, spectrally decompose metabolites, assess blood flow, measure tissue stiffness,
and more. These different types of image contrasts play an important role in diagnostic
imaging and neuroscience, and each is realized by carefully manipulating a large number of user controls
during the scan.

Despite the benefits, long scans times remain a major limitation. A typical MRI
scan takes about 5 minutes; in comparison, a full-body computed tomography scan takes a few seconds. To
lower scan time, concessions are often made in the acquisition process, leading to
reduced imaging resolution, image blurring, and lower signal to noise ratio (SNR). Since data collection in MRI consists of
Fourier sampling, these tradeoffs can be understood from a signal processing perspective: scan time and SNR are proportional
to the number of Fourier measurements collected, and sampling theory dictates resolution and field of view (FOV).

A recent trend for faster scanning is to leverage computational methods in order to reduce the required number of samples for reconstruction. One established technique is parallel imaging \cite{bib:pruessmann1999ys,bib:yingspm}, which takes advantage of multiple receive coils placed around the object to acquire data in parallel. Parallel imaging has become routine in clinical applications.
Another avenue that is especially suited to MRI is compressed sensing (CS) \cite{bib:lustig2008pe}. In CS MRI, data are acquired below the Nyquist rate using an incoherent measurement scheme such as pseudo-random sampling. A non-linear reconstruction then leverages image structure such as sparsity and low rank to recover the image as if it were sampled at the Nyquist rate.

While extremely powerful, these image priors are phenomenological in nature, and do not account for the mechanism behind the image formation. On the other hand, the MRI physics provide explicit knowledge of the signal behavior. By accounting for the signal dynamics, it is possible to jointly design new sampling schemes and reconstructions that further constrain the space of solutions beyond sparsity based on image content alone. In this article, we provide an overview of CS MRI incorporating physics-based constraints, and show how it can be used to accelerate acquisitions, eliminate artifacts, and extract quantitative bio-physical information from the scan. We limit our scope to spin density and relaxation effects, though in general the concepts apply to other intrinsic tissue parameters \cite{CITATION}.

\section{MRI Background}
\subsection{MRI Physics}
The MRI system can be approximated by a discrete linear dynamical system based on the Bloch equations, shown in \autoref{fig:mri_dynamical_system}. An aggregate of spins in each 3D spatial position (called a voxel) creates a net magnetization that is initially aligned with MRI's strong magnetic field, and evolves based on intrinsic biophysical tissue parameters and user control inputs consisting of radio-frequency (RF) and magnetic field pulses. RF pulses act to rotate or \textit{excite} the magnetization vector away from the main field direction, effectively mixing its longitudinal and transverse components. 
The strength and duration of the RF pulse determines the degree of rotation, or \textit{flip angle}, experienced. The transverse component of the magnetization is sensed by nearby receive coils through Faraday's Law.
\myfig[mri_dynamical_system]{The MRI dynamical system. An aggregate of spins at each voxel position creates a net magnetization that evolves based on user pulse sequence control inputs and intrinsic tissue parameters.}

When no control inputs are played, the magnetization will return to the equilibrium state at a rate governed by the tissue's relaxation parameters. The longitudinal component will exponentially recover to its initial state with time constant \Tone, and the transverse component will exponentially decay to zero with time constant \Ttwo.
As \autoref{fig:Bloch_Toilet} shows, relaxation can be understood through analogy with a toilet, where the water in the tank represents longitudinal magnetization, water in the bowl represents transverse magnetization, and the toilet flush is an RF waveform generator. When the toilet is flushed (excitation), water transfers from the tank to the bowl, producing a detectable signal. As the toilet bowl drains (\Ttwo relaxation), the tank refills with water (\Tone recovery). Successive flushes will transfer new water from the tank to the bowl.
Neglecting other system effects, the magnetization is given by
\begin{align}
  M_z(t) &= M_0\left( 1 - e^{-\frac{t}{T_1}}\right), \label{eqn:t1} \\
  M_{xy}(t) &=  M_{0}e^{-\frac{t}{T_2}} \label{eqn:t2},
\end{align}
where $M_{z}(t)$ and $M_{xy}(t)$ are the longitudinal and transverse magnetization components at time $t$ after the excitation, respectively, and $M_{0}$ is the magnetization at thermal equilibrium.

\myfig[Bloch_Toilet]{Signal relaxation visualized through the toilet analogy. The longitudinal and transverse time constants, referred to as \Tone and \Ttwo, respectively, are intrinsic physical parameters and differ across tissue types.}

In general, the transverse magnetization can be described by
\begin{align}
  M_{xy}(\vec r, t) = \rho(\vec r)f_t(\vec{r}),
  \label{eqn:mri:mxyt}
\end{align}
where $\rho(\vec r)$ is the intrinsic amount of magnetization at position $\vec r$ (called proton-density, or PD), and $f_t(\vec r)$ is a spatio-temporal signal evolution that depends on the tissue and pulse sequence parameters.
By manipulating the sequence controls and sampling the magnetization at appropriate times, many different types of image contrasts can be captured. \autoref{fig:brain_multicontrast} shows four common image contrasts based on PD, \Tone, and \Ttwo.
\myfig[brain_multicontrast]{Image contrasts based on PD, \Tone, and \Ttwo produced by manipulating pulse sequence timing.}

\mysubsection{Frequency Domain Formulation}
The MRI signal samples spatial frequencies of the transverse magnetization, and the linear relationship is described by the integral 
\begin{align}
  s(t) = \int_{\vec r} M_{xy}(\vec r, t) e^{-j 2 \pi \vec{k}(t)^\top\vec r} d\vec{r} + w(t),
  \label{eqn:mri:signal_equation}
\end{align}
where $s(t) \in \mathbb{C}$ is the acquired signal at time $t$ after the RF excitation, $M_{xy}(\vec{r}, t)$ is the transverse component of the magnetization that depends both on spatial position $\vec r$ and time $t$, $\vec{k}(t)$ is a trajectory of 3D frequency points and $w(t)$ is complex-valued white Gaussian noise. The symbol $(\cdot)^\top$ is used to denote the transpose operation.
Because the spatial frequency points are denoted as $\vec k$, MRI acquisition is often described as sampling in \textit{k-space}.
After change of variables and discretization, the MR signal equation is represented as the linear operator
\begin{align}
  \vec y = \vec{E x} + \vec w,
  \label{eqn:forward_model}
\end{align}
where $\vec x \in \complex{N}$ is the image, $\vec y \in \complex{M}$ are the acquired data in k-space, $\vec E \in \complex{M\times N}$ represents the spatial encoding, and $\vec w \in \complex {M}$ is noise.
If each measurement is acquired at time $t=\mathrm{TE}$ (called the \textit{echo time}) after RF excitation, temporal magnetization effects can be ignored and the forward model is
\begin{align}
  \vec E = \vec{PF},
  \label{eqn:forward_model_simple}
\end{align}
where $\vec F$ is a Fourier transform operator and $\vec P$ is the operator that selects the acquired k-space samples.
\autoref{fig:forward_model} illustrates this forward model relationship. In the case of 3D Cartesian imaging, the acquired samples are represented as points on a 2D grid, though more complicated, non-Cartesian sampling trajectories are also possible \cite{NONCART}.

\myfig[forward_model]{The discretized MRI forward model given by $\vec y = \vec{PFx}$. The MR image is Fourier transformed and measurements are acquired in k-space. In the case of 3D Cartesian imaging, the acquired samples are represented as points on a 2D grid.}

It is common to receive the MRI signal in parallel from multiple receive coils placed around the object. In particular, each coil element is sensitive to a local region of the underlying object, and can be represented as the underlying image multiplied with spatially varying coil sensitivity maps. Concretely, with multi-channel coil arrays, $\vec y \in \complex{CM}$ consists of multiple measurement vectors
\begin{align}
  \vec y_j = \vec{PFS}_j \vec{x} + \vec w_j, \quad j=1,\dots,C
  \label{eqn:forward_model_multicoil}
\end{align}
where $\vec S_j \in \complex{N\times N}$ is a diagonal matrix with the spatial sensitivity values on the diagonal, and $\vec w_j \in \complex{M}$ is the noise at the $\nth{j}$ coil, respectively, and $C$ is the number of coil elements in the array. Because the received signals are acquired in parallel, the sampling operator $\vec P$ is shared among all the channels. Parallel imaging uses the multi-channel measurements to under-sample k-space while maintaining a well-posed reconstruction.

\subsection{Signal Dynamics}
For many applications, it is not practical to wait for relaxation effects to ``reset'' the spin system before acquiring each measurement, as the effective wait time or \textit{repetition time} (TR) can be multiple seconds. This would translate to hundreds of hours of scan time. To overcome this limitation, several samples can be collected in a single TR to accelerate the acquisition. This is the basis of the RARE technique \cite{bib:hennig1986}, also known as fast spin-echo (FSE) or turbo spin-echo (TSE). However, the transverse magnetization evolves while sampling, breaking the simple Fourier transform relationship.
When left unmodeled, the signal dynamics modulate the acquired data and cause an undesirable filtering effect on the image. In the case of FSE, this leads to spatially varying image blurring due to \Ttwo relaxation, shown in \autoref{fig:fse_blurring}.
\myfig[fse_blurring]{Effects of collecting samples at multiple TEs with FSE. (left column) A 90$^\circ$ excitation pulse (red rectangle) followed by 180$^\circ$ refocusing pulses (gray rectangles) will lead to exponential decay due to \Ttwo relaxation. (middle column) When a single sample is acquired in each TR duration (red circles), a sharp image can be reconstructed. To accelerate the acquisition, measurements can be acquired between each refocusing pulse, shown as digital-to-analog (DAC) blocks. However, k-space will be modulated by \Ttwo relaxation based on its acquisition time (multi-colored circles), leading to image blurring (right column). Since \Ttwo depends on position, each voxel will exhibit different amounts of blurring.}

The linear forward model can be extended to represent the signal dynamics in the FSE experiment by including additional image states, $\vec x = \begin{bmatrix} \vec x_1 & \cdots & \vec x_T \end{bmatrix}$, where $\vec x_i \in \complex{N}$ is the image at the $\nth{i}$ imaging time and $T$ is number of time points. The forward model, illustrated in \autoref{fig:temporal_forward_model}, includes different encoding operators for time point $i$ and coil $j$:
\begin{align}
  \vec E_{ij} = \vec P_i \vec F \vec S_j.
  \label{eqn:temporal_forward_model}
\end{align}
The same concept can be used to include additional dimensions such as motion states due to cardiac or respiratory motion \cite{bib:lustig2007hl,bib:jiang2018pe}, spectral states for MR spectroscopy, dynamic contrast enhancement states \cite{bib:feng2014sm,bib:zhang2015iq}, and many others.
  \myfig[temporal_forward_model]{The forward model extended to relaxation dynamics for FSE. Each image represents an sampling time during the FSE acquisition, $T=4$ time points in this example. The forward model includes the sensitivity map operator ($C=2$ channels), the Fourier transform, and sampling. Each time point can be sampled differently, for instance using a center-out ordering of k-space.}

In the following sections, we see how modeling the signal dynamics allows us to reduce these artifacts as well as solve for the intrinsic tissue parameters that govern the dynamics.


==> old_2_imaging_system_design.tex <==
\section{Pulse Sequence Design}\label{subsec:system_design}
Designing an MRI pulse sequence consists of two main components: (\textit{i}) designing the pulse waveform and timing to guide the signal evolution, and (\textit{ii}) designing the spatial encoding to appropriately sample k-space. Initial work focused on designing sequences with simple goals in mind such as maximizing contrast and limiting blurring \cite{bib:mugler2014gc}. A recent trend in computational MRI approaches is to use optimal experiment design to motivate scan parameter selection \cite{TODO}, and incoherent sampling properties to motivate k-space sampling \cite{bib:lustig2008pe}. Importantly, both should be designed with a specific reconstruction in mind. Although optimal experiment design in principle can be applied to spatial encoding as well, it leads to a prohibitively expensive optimization and remains an unexplored area of study. More recently, data-driven approaches that optimize (\textit{i}) and (\textit{ii}) jointly or separately have shown promise at achieving this goal.

\subsection{Sequence Parameter Selection}
The classical approach to creating signal contrast between different tissue types is to choose a specific imaging time that maximizes the difference in signal value between two target species. For example, focusing on \Ttwo contrast given by \autoref{eqn:t2}, and defining the signal difference between two tissue species $A$ and $B$ as $M_{xy, A}(t) - M_{xy, B}(t)$, the imaging time that maximizes the difference is given by 
\begin{align}
    t^\star = -\frac{\log\left(\frac{T_{2,A}}{T_{2,B}}\right)}{\frac{1}{T_{2,A}}-\frac{1}{T_{2,B}}}.
    \label{eqn:cnr}
\end{align}
The same concept is used to null tissue signal in inversion recovery sequences based on \Tone (\autoref{fig:brain_multicontrast}).

Under the multiple measurement model \autoref{eqn:temporal_forward_model}, when multiple time points need to be chosen, an alternate formulation based on optimal experiment design is to maximize sensitivity to a particular parameter.

T1, T2 parameter maps are very useful biomarkers in monitoring the progression of various neurological and cardiac disorders.
Classical sequences such as inversion/saturation (IR/SR) or spin echo methods provide simple and reliable methods for estimating T1 and T2 maps, however, are limited by their long repetition time (TR).
On the other hand, steady-state sequences such as dual-echo steady-state (DESS) and Spoiled Gradient-Recalled Echo require a much shorter TR, greatly reducing scan time, and are sensitive to T1 and T2 variation. However, the T1, T2 cannot be directly extracted from the resulting signals requiring multiple acquisitions with different parameter sets to obtain T1, T2 maps.

Nataraj \textit{et al.} provide a general framework to optimize the sequence parameters (TR, TE and flip angle) of combinations of pulse sequences in order to provide accurate and precise parameter maps. 
Inspired by the Cramer-Rao Bound (CRB), which bounds the minimum variance of an unbiased estimator, the set of scan parameters are optimized to minimize the worse-case maximum cost. The constructed optimization problem is solved with grid search.
The method is demonstrated on T1, T2 estimation from a 3 sets of different combinations of DESS and SPGR scans.
Numerical simulation results for optimized scan parameters of the 3 sets of combinations demonstrate that precise T1 and T2 parameters maps can be obtained.
Although the optimized scan profiles consisting of a combination of SPGR and DESS scans yield accurate results for the phantom dataset, these results do not hold up for the in vivo datasets, unless scan time is increased further.

Gradient-echo sequences can allow for faster acquisitions, however, after the preparation module signal decays gradually resulting in the initial contrast being reduced to a lower steady-state contrast level.
Two techniques to tackle this issue are segmented k-space acquisitions where a preparation module is repeated at the start of each segment, at the expense of longer scan times, and centric phase-encode ordering where low frequencies are acquired first after preparation, which results in reduced image resolution as higher spatial frequencies experience signal decay. This results in a tradeoff between image contrast and scan efficiency. 

Cukur \textit{et al.} combine a post processing technique with centric phase-encode ordering and apply it to magnetization-prepared steady-state free precession (SSFP) angiography which improves contrast with no increase in scan time. The technique is based on the fact that in lower-extremity angiograms, the background mainly consists of skeletal muscle tissue with relatively lower spatial frequency content and the tissue of interest is thin blood vessels that have higher spatial-frequency content.
A compensation filter inversely proportional to the level of magnetization of the blood vessels is applied the acquired signal in the frequency domain, which compensates for the signal decay in blood vessels with no significant effect on the background muscle signal.
The compensation filter is combined with a sparsity-enforcing compressed sensing (CS) reconstruction, which can reduce the increased image noise due to the increased weighting of the higher spatial frequency components as a result of the compensation filter.
The highly compressible angiographic dataset is sampled with a variable-density random undersampling pattern in the k-space with decaying probability density towards higher spatial frequencies. The reconstruction is performed by solving a unconstrained nonlinear optimization problem that simultaneously enforces that the resulting reconstructed image is compressible and consistent with the acquired data.

Rapid Acquisition with Refocused Echoes (RARE) imaging uses an echo train consisting of echoes with changing phase encoding gradient allowing multiple lines in the k-space to be acquired in a single repetition time (TR). This sequence demonstrates that refocusing flip angles can be used to produce a higher signal intensity than the first echo as a result of constructive interference. 
Busse \textit{et al.} present a technique to optimize the flip angles of the echo train to increase signal-to-noise ratio (SNR) of the resulting signal and produce a modulation transfer function (MTF) for different materials that improves resolution.
In addition they calculate a “contrast-equivalent” TE for each echo in the train, that matches the contrast that would have been achieved by a single echo, and show that the image contrast can be manipulated.
 The method proposed by the paper uses the inverse of the EPG algorithm ("Prospective EPG Algorithm") to find a sequence of flip angles that quickly establish psuedosteady-state, then keep the signal level at a constant rate for a certain number of echoes and finally start increasing the flip-angle linearly until the maximum flip angle is achieved. 
In order to rapidly establish pseudosteady-state, a signal target for each echo in the echo train is determined that asymptotically approaches the signal target, $S_{target}$. This asymptotic technique can maintain a greater signal level and requires less RF power compared to alternatives including having a constant signal level starting from the first echo or using constant flip angle until maximum signal is achieved.
Other alternatives to increasing the flip angle linearly are considered including a Gaussian and half-exponential profile, however, the varying the angle linearly was able to best satisfy the resolution and SNR requirements. This technique shows that the flip angles of the echo train can be optimized to improve SNR and limit blurring artifacts due to relaxation of different materials.

Selective-inversion-recovery (SIR) is an imaging method that measures the quantitative magnetization transfer (qMT) or spin exchange between protons in free water and macromolecules by applying an RF pulse that selectively inverts the protons in free water. 
The precision and accuracy of the qMT measurements from a SIR sequence depend on several parameters including the inversion recovery time ($t_i$) and the predelay time ($t_d$).
The signal measured by the SIR sequence can be expressed as a function of qMT parameters by adding the coupling between different pools to the Bloch equations.
Li \textit{et al.} introduce a CRLB based optimization technique that varies both $t_i$ and $t_d$ sampling points in order to maximize the qMT and T1 measurement precision efficiency separately for the worse case combination of parameters. Monte Carlo simulations are also performed by adding Gaussian noise to measure the uncertainties of the optimized parameters.
The results show that higher precision efficiencies can be obtained for both T1 and qMT measurements compared to previous methods and the uncertainties of the fitted parameters are reduced.


\subsection{Trajectory/Acquisition Strategies}


Various trajectory/acquisiton strategies have been explored to find the optimal k-space trajectory for a given task. Halder \textit{et al.} formulate an exponential decay based parametric contrast model of an image sequence consisting of $L$ different frames acquired with different image acquisition parameters. Each frame is thus a different contrast modulation of the same underlying image image. They examine the best trajectory in order to achieve high-resolution image frames as well as parameter maps. Both a CRB-based theoretical analysis as well as phantom experiments are performed to compare several 2D Cartesian sampling schemes and determine which scheme yields the most accurate reconstruction. 


Lustig \textit{et al.} determine a more efficient k-space trajectory by employing the fact that the MR image has transform sparsity, a sparse representation in a fixed mathematical transform domain.
If an image exhibits transform sparsity, and if undersampling in the frequency space results in incoherent artifacts in the image space, then the image can be recovered from the undersampled frequency space data with a nonlinear recovery method. 
The sparsity of MR images are displayed by performing a sparsifying transform on fully sampled images and reconstructing the images from various subsets of the largest transform coefficients.
Transform Point Spread Function (TPSF), which determines the contribution of one transform coefficient to another transform coefficient, was used to measure the incoherence of the sampling trajectory. 
A sampling pattern can be determined by a Monte-Carlo design procedure where you determine a variable density pattern obtained by randomly drawing indices using a probability density function, calculate the TPSF of the obtained trajectory and repeat the procedure several times. Choose the pattern with the lowest peak interference. 
The reconstruction is performed with a constrained optimization problem that involves maximizing the sparsity of the reconstructed image (using the l1 norm of the sparsifying transform of the image) while having a constraint that enforces data consistency. \textbf{add equations here} An additional Total Variation term can be added to the objective which enforces the sum of absolute variations in the image to be smaller. This allows the image to be sparse in the transform space and by finite differences simultaneously.


Building on (cite SPARSE MRI), OEDIPUS is a principled method for designing sampling patterns for sparsity-constrained MRI which accounts for coil geometry, anatomy, image contrast and can be reused for different subjects.
OEDIPUS uses a design based on the CRB bound on the covariance of an unbiased estimator. The CRB-based design for a unconstrained linear model, $d=Af+n$ where $f \in \mathbb{C}^N$, is modified by informing the model that the image vector has a certain level of sparsity, i.e. $\norm{\Psi f}_{0}\leq S$ where $\Psi \in \mathbb{C}^{Q \times N}$ is a known sparsifying transform and $S$ is the sparsity level. The linear model can then be written as $d=A \Psi^{\dagger} U\widetilde{c}+n$. Here, $c=\Psi f \in \mathbb{C}^Q$ and $c=U\widetilde{c}$ where $\widetilde{c}$ contains the S nonzero entries of $c$ and $U$ is a matrix formed by concatenating the $S$ columns of a $Q \times Q$ identity matrix. 
The CRB bound for the covariance matrix of the unbiased matrix in the linear model is 

\begin{equation*}
    cov(\hat{f}(d)) \succeq (A^HA)^{-1}
\end{equation*}

The model, informed of the sparsity constraints becomes

\begin{equation*}
    cov(\hat{f}(d)) \succeq \Psi^{\dagger}U(U^H(\Psi^{\dagger})^HA^HA\Psi^{\dagger}U)^{-1}U^H(\Psi^{\dagger})^H
\end{equation*}

The addition of the sparsity constraint also leads to large computational complexity advantages since the expressions being inverted are only size $S \times S$.
CRB bound considered in the paper is only valid for unbiased estimators, however, the problem at hand is not necessarily unbiased.


==> old_3_physical_modeling.tex <==
\section{Physical modeling}\label{sec:physical_modeling}
\comment{Ke \\
This section will discuss low-dimensional modeling based on the physical properties of the signal. The section will focus on linear subspace design informed by the expected behavior of the signal given the system design in Section~\ref{subsec:system_design} \cite{bib:zhao2012,bib:huang2012,bib:huang2013,bib:velikina2013}.
}
As the MRI signal is generated by protons in the body under a strong static magnetic field $B_0$, the signal itself is constrained by nuclear magnetic resonance physics like radio frequency (RF) excitation and relaxation. In this regard, the physics properties of the signal can be leveraged for low-rank modeling and image reconstruction. Conventional imaging methods assume that the samples of the frequency domain $s(\textbf{k},t)$ has to satisfy Nyquist rate. However, it has been demonstrated that high-quality images can be reconstructed from undersampled k-space data with appropriate physics constraints. These constraints include partial separability and sparsity for dynamic imaging reconstruction\cite{bib:zhao2012}, low-rank model for relaxation estimation\cite{bib:huang2012,bib:t2shmethod}, the smoothness in the parametric dimension and the relevant reconstruction methods\cite{bib:velikina2013}.

On the other hand, by utilizing the physics model behind MRI using the Bloch Equation\cite{bib:bloch1946nuclear}, we can design powerful simulator tools for MR signal simulation, which can be used for optimizing scan parameters and sequence programming. Some useful simulator will be briefly discussed in this section. Additional modeling approaches, including union of subspaces \cite{bib:velikina2015reconstruction,Mandava:MagnResonMed:2018}, low-rank tensors \cite{bib:christodoulou2018} and manifold learning \cite{bib:nakarmi2017}, will be briefly introduced.
\subsection{Physics Model for Image Reconstruction}
For traditional imaging methods, Nyquist sampling rate in the frequency domain is required for image reconstruction. However, the signal evolution function of MRI follows physics model(bloch equation\cite{bib:bloch1946nuclear}) which can be used for a low-dimensional representation of the signal itself. With some physics based assumptions or
constrains, image reconstruction for dynamic imaging, quantitative mapping and multi-contrast imaging can achieve a higher undersamping rate. Among them, Zhao \textit{et al.} proposed a dynamic image reconstruction method from highly undersampled (\textbf{k},\textit{t})-space data to use partial separability (PS) and sparsity constraints jointly for real-time cardiac MRI\cite{bib:zhao2012}. The proposed model incorporates the complementary advantages of both PS and sparsity constrains into a single formulation by using sparsity constraint on PS regularization, which is shown as follow:
\begin{equation}
\hat{\vec{\rho}} = \arg \min_{\bm{\rho}\in \mathbb{C}^{NM \times 1}}\| \bm{d}-\bm{\Phi \rho}\|_2^2+R_r(\bm{\rho})+R_s(\bm{\rho}),
\end{equation}
where $\vec{d}\in\mathbb{C}^{D\times 1}$ contains the measured data, $\bm{\Phi}\in\mathbb{C}^{D\times NM}$ is the measurement matrix, consists of the spatial Fourier Transform and sparse sampling operator. $\bm{\rho}=\text{vec}(\bm{C})\in \mathbb{C}^{NM\times1}$ is the matrix and vector representation of the dynamic image $\rho(x,t)$. The penalty function $R_r(\cdot)$ and $R_s(\cdot)$ are used to incorporate the PS and sparsity constrains respectively.
Also, a globally convergent computational algorithm is described to solve the underlying optimization problem. By using these properties of the signal, the in-vivo experiments demonstrated the better performance than using partial separability and  sparsity constraints individually, and can be applied to more dynamic imaging applications.

Besides the dynamic imaging, physics model based reconstruction algorithm can also be incorporated to quantitative parameter mappings (T1, T2 mappings).Huang \textit{et al.} presented a model-based algorithm to reconstruct T2 mapping from highly undersampled data, by combining principal component analysis. The nonlinearity related to T2 estimation is remove by introducing PCA where the exponential decay can be accurately approximated by linear combination of a few pre-calculated principal components (PCs). To be more concrete, let $\overrightarrow{v}$ be a real vector representing a noiseless exponential $T_2$ decay curve for real $I_0$ values, the exponential decay model can be wriiten as:
\begin{equation}
    v_j=I_0\cdot \text{e}^{-TE_j/T_2}.
\end{equation}
Let $L$ be the number of principle components, the $T_2$ decay curve can be approximated by the linear combination:
\begin{equation}
    \overrightarrow{v} = \sum_{i=1}^{L}m_i\overrightarrow{b_i}+\overrightarrow{\epsilon},
\end{equation}
where $\overrightarrow{b_i}$ is the $i$th PC vector and $m_i$ is the corresponding weights.
Following this work, Huang \textit{et al.} further developed an algorithm for fast and accurate T2 estimation from highly undersampled multi-echo spin-echo data, leveraging a model-based reconstruction method based on slice-resolved extended phase graph (SEPG) model. The principal components (PCs) are calculated for given TE points using a training set of decay curves given by SEPG model. Also,Velikina \textit{et al.} proposed an accelerating MR parameter mapping using sparsity-promoting regularization in parametric dimension. The signal in the parametric dimension is described by a smooth function, which is viewed as a regularization term in a CS-type minimization problem. The images series obtained as the solution of this minimization problem is then fit to a parametric model to yield parameter maps.


\comment{Approaches to simulating the signal will be discussed, including Bloch Simulation \cite{bib:eliezer2014} and the Extended Phase Graph Algorithm \cite{bib:weigel2015}.}

\subsection{MR Signal Simulation tools}
In the past decades, approaches to simulate the MR signal has been well developed based on the physics models, including simulators based on Bloch equations\cite{bib:bloch1946nuclear} and the Extended Phase Graph\cite{bib:weigel2015}. As the fundamental physics model of NMR and MRI, the Bloch equations are a set of macroscopic equations used for calculating the nuclear magnetization as a function of time when relaxation times are present. By leveraging Bloch simulation, Ben-Eliezer \textit{et al.} presented a postprocessing approach to overcome the common penalties associated with multiecho protocols. Bloch simulations are repeated for a range of $\text{T}_2$ values and transmit field scales, yielding a dictionary of simulated echo-modulation curve (EMC), which is then used to determine the $\text{T}_2$ value by finding the most closely matches curve in the dictionary.

The extended phase graph is a powerful tool for simulating and understanding the magnetization response of MR sequences. The effect of gradients, radiofrequency (RF) pulses, relaxation, and motion phenomena during the MR sequence is characterized as the action of a few matrix operations on different magnetization states, which can be viewed as a useful tool for MRI sequences design.

\textbf{Figure 1} Show an example of how EPG works. Using the Fig 3 in the paper may be an option.


\subsection{Additional  Modeling  Approaches}
Besides the methods introduced in the previous section, additional modeling approaches, including union of subspaces \cite{bib:velikina2015reconstruction,Mandava:MagnResonMed:2018}, low-rank tensors \cite{bib:christodoulou2018} and manifold learning \cite{bib:nakarmi2017}, will be briefly introduced in this section. By leveraging the consistency in the temporal domain, Velikina \textit{et al.} introduced the model consistency condition (MOCCO) technique, utilizing temporal models to regularize reconstruction without constraining the solution to be low-rank\cite{bib:velikina2015reconstruction}.

\textbf{Figure 2} Show how mocco works, cite maybe fig 7 in the paper.

This method allows enforcing consistency with the data-driven pre-estimated model, which can improve the reconstruction of dynamic imaging. Following this method, Mandava \textit{et al.} presented an extension of the MOCCO framework to work with a union of local subspaces constraint for quantitative mapping. Magnetic resonance multitasking conceptualized different sources of image dynamics as different time dimensions, using a low-rank tensor (LRT) imaging method for cardiovascular imaging. Christodoulou \textit{et al.} developed a new LRT imaging strategy, where a factored tensor reconstruction approach that enforces the LRT in two efficient steps. Nakarmi \textit{et al.} proposed a novel kernel-based framework to learn and incorporate a nonlinear manifold into constrained reconstruction from reduced acquisition by using kernel principal component analysis (KPCA).



==> old_4_constrained_image_reconstruction.tex <==
\section{Physics Constrained Image Reconstruction}
\comment{Frank
This section will describe a generalized inverse problem that captures both physics-based structure and image-based prior knowledge \cite{bib:csmri,bib:doneva2010,bib:zhao2014}. Different formulations will be described along with their tradeoffs, e.g.\ explicit constraints vs regularization, and their effects on physical parameter estimation.}

Given the acquired k-space measurements $\{\vec{y}_{ij}\}_{ij}$, there are in general two goals: one is to reconstruct the underlying image sequence $\{\vec{x}_j\}_j$, and the other is to recover the quantitative parameter maps $\vec{T}_1$ and $\vec{T}_2$. \TODO{rephrase}Certain applications, such as in musuclar skeletal imaging, desire the image sequence of different contrast for better visualization, while other applications, such as in cardiac imaging, wants the quantitative maps.  In this section, we will focus on image reconstruction.

Because of long acquisition time, it is desirable to shorten the number of samples. Such inverse problems are in general ill-posed and physical-based structures and image-based prior knowledge are used to help regularize the recovery problem.

Various works have been proposed and in general consider objective functions of the following form:
\begin{equation}
\begin{aligned}
  &\underset{\vec{x}}{\text{minimize}}~\frac{1}{2} \sum_{i = 1}^T \sum_{j} \| \vec{E}_{ij} \vec{x}_j - \vec{y}_{ij} \|_2^2 + \lambda \mathcal{R}(\vec{x})\\
  &\text{subject to}~\vec{x} \in \mathcal{C}
\end{aligned}
\end{equation}
where $\mathcal{C}$ is some physics-based constrained set, and $\mathcal{R}$ is some regularization function.


\myfig[physical_constraint]{Physics-based constraints}

One way of utilizing the physical forward model is to enforce the underlying image to lie on the exact physical constraint:
\begin{equation}
\begin{aligned}
  \mathcal{C} = \{[\vec{x}_1(T_1, T_2), \hdots, \vec{x}_T(T_1, T_2)] : (T_1, T_2) \in \mathbb{R}_+^2\}
\end{aligned}
\end{equation}


But there are a number of difficulties. First the set is non-linear and non-convex. Second, any systematic error in the forward model would cause huge errors in the result. Highly coherent. Hence, in practice, the . However for simple systems, there are some works. \TODO{Related works}. 

Instead of computing the forward model explicitly, low-rank approaches can be used to reduce computation. Low-rank approaches rely on a partial separability model \cite{bib:zhao2012}: there is strong spatiotemporal correlation in the data between, for example, frames of a dynamic image. The model of $L^{th}$ order partial separability for dynamic imaging is:
\begin{equation}
s(k_x, k_y, k_z, t) = \sum_{l=1}^{L}{g_l(k_x,k_y,k_z)h_l(t)}
\end{equation}
where $h_l(t)$ are the temporal bases and $g_l$ are the spatial bases. 
The acquired data can be stacked into a Casorati matrix that indexes over k-space and time. In undersampled acquisitions, this matrix will have missing entries. The goal is to fill in the missing entries of the Casorati matrix $C$ subject to $rank (C) \leq L$. 
\textbf{Figure 2}: show the Casorati matrix (see googledoc).

This model becomes very useful for spatially and temporally incoherent acquisitions, such as Magnetic Resonance Fingerprinting.


Single evolutions can be simulated using the Bloch equation or EPG as described in Section~\TODO{section}. In particular, given an ensemble of spins sampled at $T$ echo times, $\vec{X} \in \mathbb{C}^{T \times N}$. 

\begin{equation}
    [\vec{x}_1(T_1, T_2), \hdots, \vec{x}_T(T_1, T_2)]
\end{equation}


\begin{equation}
\begin{aligned}
  \mathcal{C} = \{\vec{x} = \vec{\Phi}_K \bm{\alpha}\}
\end{aligned}
\end{equation}

Some image based priors to incorporate:

Wavelet/gradient sparsity prior
\begin{equation}
\begin{aligned}
  \mathcal{R}(\vec{x}) = \| \vec{\Psi} \vec{x} \|_1
\end{aligned}
\end{equation}


Low rank prior
\begin{equation}
\begin{aligned}
  \mathcal{R}(\vec{x}) = \| \vec{x} \|_*
\end{aligned}
\end{equation}




==> old_5_quantitative_mapping.tex <==
\section{Quantitative Mapping}
\comment{Suma \\
This section will show how the reconstructed data can be used to fit quantitative parameters to the physical model, e.g.\ through direct estimation \cite{bib:block2009}, non-linear least-squares, dictionary-based matched filtering \cite{bib:zhao2017,bib:asslander2017}, and novel approaches that operate directly in the low-dimensional subspace defined by the physical model \cite{McGivney:IeeeTransMedImaging:2014}. 
}

\subsection{Nonlinear least squares}
To estimate $T_1$ and $T_2$ maps, many approaches consider the reconstructed images and then fit quantitative parameters. Instead, it is possible to estimate $T_1$ and $T_2$ directly from k-space, without the intermediate step of reconstructing an image \cite{bib:block2009}. This is done via modeling the reconstruction, and solving iteratively for the parameters directly. 

As an example, for reconstructing $T_2$ and $\rho$ (proton density) maps from an undersampled fast spin echo acquisition \cite{bib:block2009}, we would like to recover the pair $(\vec{\rho}, \vec{r})$ from the raw data $\vec{y}$, where $r = 1/T_2$ for each element in $\vec{r}$. We can model $(\vec{\rho}, \vec{r})$ as a sum of scaled delta functions, where each voxel in the image is scaled by $\rho_{i}$ and $r_{i}$. Let the functions that evaluate $\rho_{i}$ and $r_{i}$ at each point in space by denoted by $\varrho$ and $R$, i.e.:

\begin{equation}
	\varrho(\vec{x}) = \sum_i{\rho_i \cdot \delta(\vec{x} - \vec{x_i})}
\end{equation}

and
\begin{equation}
	R(\vec{x}) = \sum_i{r_i \cdot \delta(\vec{x} - \vec{x_i})}
\end{equation}

We can construct the following forward model of the $j^{th}$ acquired sample as:
\begin{equation}
    F_j(\vec{\rho}, \vec{r}, t,c) = \sum_{\vec{x} \in FOV}{ \varrho(\vec{x}) \cdot e^{-R(\vec{x}) \cdot t} \cdot C_c(\vec{x}) \cdot e^{-j\vec{x} \cdot \vec{k_j}}} 
\end{equation}

where $C_c(\vec{x})$ is the coil sensitivity profile of the $c^{th}$ coil at position $x$, and $t$ indexes over echo times.

To solve for $(\vec{\rho},\vec{r})$, we can solve a nonlinear least squares objective. Generally, this is of the form:

\begin{equation}
    \theta \in \text{argmin}~\| \vec{E} \vec{x}_t (\theta) - \vec{y}_t \|_2^2
\end{equation}

In this case, the objective is:
\begin{equation}
	\Phi(\vec{\rho}, \vec{r}) = \frac{1}{2}\sum_t{ \sum_c{ \|F(\vec{\rho}, \vec{r}, t,c) - \vec{y_{t,c}} \|_2^2}}
\end{equation}

The objective can be minimized with the conjugate gradient algorithm. It is differentiable; however, it is highly nonconvex. Additionally, the solution may result in unrealistic map estimates because an area of k-space may be ill-conditioned. Therefore, regularization term $P(\vec{\rho}, \vec{r})$ can be added to ensure smoothness:
\begin{equation}
	\Phi(\vec{\rho}, \vec{r}) = \frac{1}{2}\sum_t{ \sum_c{ \|F(\vec{\rho}, \vec{r}, t,c) - \vec{y_{t,c}} \|_2^2}} + \lambda \cdot P(\vec{\rho}, \vec{r})
\end{equation}


\subsection{Dictionary matching}
Another approach is to generate a dictionary of possible signal evolutions and pattern-match the reconstructed image to it, voxel by voxel. This technique is commonly used in Magnetic Resonance Fingerprinting \cite{bib:ma2013}. In MRF, data are acquired with pseudo-random parameters such as flip angles and TRs. The trajectory is an undersampled variable density spiral so that there is both spatial and temporal incoherence, which leads to incoherent aliasing. The reconstruction estimates parameters by pattern-matching to a pre-computed dictionary, voxel by voxel. Since the signal evolutions are very similar to one another, it is possible to compress the dictionary via SVD \cite{McGivney:IeeeTransMedImaging:2014} or to solve for the spatial and temporal components directly via low-rank matrix factorization \cite{bib:zhao2017}. These approaches are not discussed in detail here, but are explained in a different article in this issue.

\subsection{Nonlinear least squares from reconstructed image}
\begin{equation}
    \theta \in \text{argmin}~\| \vec{x}(T_1, T_2) - \vec{x} \|_2^2
\end{equation}


\subsection{Dictionary matching}
\begin{equation}
    \theta \in \text{argmax}_\theta~\left< \vec{E} \vec{x}_t (\theta), \vec{y}_t \right>
\end{equation}


\subsection{Nonlinear least squares from k-space}
\begin{equation}
    \theta \in \text{argmin}~\| \vec{E} \vec{x}_t (\theta) - \vec{y}_t \|_2^2
\end{equation}























